A survey for variable young stars with small telescopes: VIII -- Properties of 1687 Gaia selected members in 21 nearby clusters

The Hunting Outbursting Young Stars (HOYS) project performs long-term, optical, multi-filter, high cadence monitoring of 25 nearby young clusters and star forming regions. Utilising Gaia DR3 data we have identified about 17000 potential young stellar members in 45 coherent astrometric groups in these fields. Twenty one of them are clear young groups or clusters of stars within one kiloparsec and they contain 9143 Gaia selected potential members. The cluster distances, proper motions and membership numbers are determined. We analyse long term (about 7yr) V, R, and I-band light curves from HOYS for 1687 of the potential cluster members. One quarter of the stars are variable in all three optical filters, and two thirds of these have light curves that are symmetric around the mean. Light curves affected by obscuration from circumstellar materials are more common than those affected by accretion bursts, by a factor of 2-4. The variability fraction in the clusters ranges from 10 to almost 100 percent, and correlates positively with the fraction of stars with detectable inner disks, indicating that a lot of variability is driven by the disk. About one in six variables shows detectable periodicity, mostly caused by magnetic spots. Two thirds of the periodic variables with disk excess emission are slow rotators, and amongst the stars without disk excess two thirds are fast rotators - in agreement with rotation being slowed down by the presence of a disk.

==> reply_to_referee.tex <==
We thank the referee for the very useful comments on our paper. We have carefully considered them and revised our paper accordingly. All changes in the paper are highlighted in bold face - except the corrected typos. Please find below our detailed response to the individual referee comments.

################################################################
Comments to the Author
Dear Authors,

I have carefully read the manuscript "A survey for variable young stars with small telescopes: VIII - Properties of 1700 Gaia selected members in 21 nearby clusters" by Froebrich et al. It is well written and deserves to be published in MNRAS after some revision. The authors analyse 1687 long term V, R, I-band light curves of young stellar objects in 21 nearby young clusters. They discuss the light curves characteristics and highlight the most common light curve types found in their sample.

I have some comments that I send below.

A general comment is that it would be important to make a figure showing light curves of different types, like symmetrical due to spots, periodic and aperiodic, dippers and bursters to illustrate your text. I also suggest that you define what dippers and bursters are.

---> Reply: All definitions for dippers, bursters, etc. are given in Sec.2.4. We note that in many cases, due to the lengths of the light curves, not much can gained from showing them (symmetric periodic and aperiodic look identical). However, we added a few examples in two figures as requested.

*Title: You actually analyse 1687 YSO instead of 1700 as said in the title.

---> Reply: Ok, we changed the title.

*Abstract: The second half of the abstract, starting from "One quarter of the stars..." should be improved to explain better the main results of your work. The sentences seem disconnected one from the other and you do not conclude much about anything. For example, what does it mean that most light curves are found to be symmetric? And the fact that dippers outnumber bursters? What type of correlation do you find between the variability fraction and the detection of inner disks? What do you conclude from the fact that two thirds of the periodic variables with disk excess emission are slow rotators?

---> Reply: The second half of the abstract was re-written to make the statements more informative and more specific.

*Sect. 2.1, 1st paragraph: Please explain why you excluded from you sample all sources with a parallax of less than 0.3 mas, a parallax signal to noise ratio below five and Gmag fainter than 18 mag.

---> Reply: We added a sentence explaining it.

*Figure 1, caption: The left panel shows the distance histogram only and not the parallax/distance histogram.

---> Reply: Correct. We deleted 'parallax/'

*Sect. 2.2, 1st paragraph: When you mention the typical seeing in the HOYS data, please state the value

---> Reply: done

*Sect. 2.2, 2nd paragraph: You say you selected all clusters that clearly showed a population of young stars. Please be more specific saying what criteria were used in this selection so that a reader can easily reproduce you work.

---> Reply: a sentence has been added.

*Sect. 2.2, 2nd paragraph: Why do you put your distance constraint at 1 kpc?

---> Reply: a sentence has been added.

*Figure 2: Please draw the extinction vector in the figure.

---> Reply: We have done that and updated the caption accordingly.

*Figure 2: I suppose all the variable stars (red dots) have HOYS light curves. So I suggest to identify them by a red open circle around the green dot.

---> Reply: Yes. We have slightly increased the symbol size and added red open circles around the variables.

*Sect. 2.3, 1st paragraph: You removed all the points that were more than 3sigma away from the median magnitude in the light curve. This could potentially remove most flares from your light curves and affect the variability analysis of you data. Can you add a figure showing an example of light curve before and after this sigma-clipping?

---> Reply: We do note that HOYS is not designed to reliably detect flares. This is pointed out e.g. in Sect.3.1.2. We do not intent to classify flare stars as bursters (even if it can happen in principle, as discussed in the text). We do not believe showing an example of a 3sigma outlier removal adds any value to the paper. Hence no such figure has been added.

*Sect. 2.3, 2nd paragraph: You say the periodograms use test frequencies between 1.3 d and the length of the light curve. However these are measures of time and not frequency.

---> Reply: Correct, we added 'one over' in both cases.

*Sect. 2.3, 4th paragraph: sigma_phot is defined twice in the same paragraph.

---> Reply: That is not the case. The first time we define what sigma_phot means and in the second sentence we state what value we have assigned to it. Anyway, we have reworded this part to avoid confusion.

*Sect. 2.3, 4th paragraph: Please show the Q values you obtained for the R filter, as you do with the M values.

---> Reply: We do no understand this comment. In this section no Q values are shown. And in all the figures we always show all the data for the R-band filter. This includes the Q-values we show in figure 4. No changes are made.

*Sect. 2.3, 5th paragraph: Please make a reference to a figure where you display the M values, like Fig. 3 for the R-band light curves.

---> Reply: We do not think such a reference is appropriate here. This is the methodology section. Fig.4, which shows Q vs M is in the results section. If we refer to this figure here, it would have to move to this part of the paper, in particular be swapped with Fig.3, and then would be several pages away from being discussed in the result section. No changes made.

*Figure 3 and Sect. 3.1.1, 1st paragraph: You say that the calculation of the M index is only meaningful for the variable stars, the ones with J larger than 1. Therefore I suggest that you should plot in grey the stars with J less than 1. Assigning a color code to them indicates that you calculated an M index value and it is misleading, since it is not meaningful.

---> Reply: Correct. We show now all the points with the corrected J value below one as gray dots in both panels.

*Figure 3 and Sect. 3.1.1, 3rd paragraph: fainter stars means G > 14 mag and bright ones mean G 10-14 mag? Please make it clear in the text. This paragraph is overall confusing, presenting a text with many repetitions.

---> Reply: In this section fainter is not specific to a particular magnitude, but is a general statement. We made this more clear in the text.

*Figure 4: Please add a scale showing the symbol size and the Stetson J index value. The left and right vertical titles refer to the same parameter, the M asymmetry index in the R band light curves, but they are called differently. Please call them by a unique name like  "R-band M Index" or "R-band M asymmetry index". Use the same name in Figure 5.

---> Reply: We have added a scale/legend to the plot and changed the y-axis label to agree with the label on the colour scale.

*Figure 5: Please add a scale showing the symbol size and the Stetson J index value.

---> Reply: That has been done in the same way as for Fig.4.

*Figure 5, caption: ...the separation between object... --> the separation between objects...

---> Reply: Fixed

*Figure 5: How do you explain the bursters (blue points) with no inner disks?

---> Reply: See the answer to the very similar comment on Sect.4 below. 

*Sect. 3.1.2, 1st paragraph: Please give a reference for the K-W2 value of 0.5 used to separate sources with and without inner disks.

---> Reply: This has been referenced a few times already in the paper, but we added a further reference here.

*Sect. 3.1.2: You discuss several morphological types of light curves but show none. It is important to show examples of the different types of light curves in the paper.

---> Reply: See the reply to the main comment above. A figure has been added.

*Sect. 3.1.3, 1st paragraph: Please, show the result of some periodogram and your light curve folded on the measured period.

---> Reply: We added one such example. 

*Sect. 4, 4th paragraph: Quasi-periodic light curves are less common than what?

---> Reply: We reworded this.

*Sect. 4, 5th paragraph: How are bursters and dippers produced in a non disk excess YSO?

---> Reply: Non K-W2 excess only means dust depletion in the inner disk. There can be colder dust further out and gas in the inner disk. We added an explanation.

*Appendix A: Please always cite the evolutionary model used when you compare your data with isochrones.

---> Reply: We have added a general note with a reference at the start of the Appendix.

*Typo: Mry --> Myr

---> Reply: Fixed
